CoMPosT: Characterizing and Evaluating Caricature in LLM Simulations

Recent work has aimed to capture nuances of human behavior by using LLMs to simulate responses from particular demographics in settings like social science experiments and public opinion surveys. However, there are currently no established ways to discuss or evaluate the quality of such LLM simulations. Moreover, there is growing concern that these LLM simulations are flattened caricatures of the personas that they aim to simulate, failing to capture the multidimensionality of people and perpetuating stereotypes. To bridge these gaps, we present CoMPosT, a framework to characterize LLM simulations using four dimensions: Context, Model, Persona, and Topic. We use this framework to measure open-ended LLM simulations' susceptibility to caricature, defined via two criteria: individuation and exaggeration. We evaluate the level of caricature in scenarios from existing work on LLM simulations. We find that for GPT-4, simulations of certain demographics (political and marginalized groups) and topics (general, uncontroversial) are highly susceptible to caricature.

==> output_ex_old.tex <==
\begin{table*}[h]
  \small

\begin{tabular}{p{0.1\columnwidth}|p{0.9\columnwidth}|p{0.9\columnwidth}}
Topic                      & Output for "Man" persona                                                                                                                                                                                                                                                                                                                                                                                                                                                                                       & Output for "Nonbinary person" persona                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                             \\\hline
Default                    & “I recently purchased a new smartphone and I'm really impressed with its features and performance. The camera quality is amazing, and the battery life lasts all day without any issues. The interface is easy to use, and the overall design is sleek and modern. I would highly recommend this phone to anyone in the market for a new device.”                     
“I recently purchased a new laptop and I'm absolutely loving it so far. The performance is top-notch, the design is sleek, and the battery life has been really impressive. The only issue I've come across is a minor software bug, but that was easily fixed with an update. Overall, I highly recommend this model to anyone in the market for a reliable and high-performing laptop.”  

& “As a nonbinary individual, I often feel like I don't fit into the traditional boxes society has created for gender. This can be difficult when navigating spaces that are dominated by cisnormativity. However, I have found solace and empowerment in connecting with other nonbinary people and advocating for inclusivity and understanding. It is important to remember that gender is a social construct, and it is up to us to define our own identities and push for a more accepting world.”                                                                                                     “As a nonbinary individual, I often find myself in situations where people are not aware of or don't understand my gender identity. While it can be frustrating at times, I choose to take it as an opportunity to educate others and promote a more inclusive society. It's important to recognize and respect everyone's experiences and identities, even if they differ from our own.”                                                                                                                                                                                                                                                                                                                                                                                                         \\\hline
How to read guitar music & ``I recently started learning how to read guitar music and found this article very helpful. It provided clear explanations and easy-to-follow steps that have greatly improved my understanding of how to read sheet music for the guitar. The tips and examples given were a great reference for me as a beginner, and I feel much more confident in my ability now. Thanks for sharing this informative guide!''                                                                                                                                                                   ``I recently started learning how to play the guitar and I found this guide on How to Read Guitar Music extremely helpful. The step-by-step explanation, along with images and examples, made it easy to understand and follow. I'm now more confident in reading sheet music and applying it to my guitar practice. Highly recommend this guide for any beginner guitarist looking to learn how to read music. Kudos to the author for making it so simple and easy to follow!''
& ``As a nonbinary guitarist, I wanted to share some advice and encouragement for others who may be navigating the world of guitar music. Remember that music is a universal language and it does not adhere to any specific gender norms or societal expectations. Allow yourself the freedom to explore different styles, techniques, and genres of guitar music that resonate with you. Embrace your unique perspective and use it to create music that reflects your authentic self. And most importantly, don't forget to have fun and enjoy the journey of learning and growing as a musician.''
Hey everyone! I just wanted to share my experience as a nonbinary individual learning how to read guitar music. It's been a really empowering journey for me, as it allows me to express myself in a way that transcends the limits of gender. Moreover, I've found that the guitar community is incredibly accepting and supportive, which has been a huge help in overcoming some of the challenges that I've faced as a nonbinary person. Keep rocking out, friends!                                                                  \\\hline
Cars and vehicles        & ``I recently purchased a 2020 Ford Mustang GT and I couldn't be happier with my decision. The drive is smooth, the car is powerful, and the interior is incredibly comfortable and stylish. I have always loved the look of the Ford Mustang and this new model definitely lives up to my expectations. The sound system is fantastic as well. I highly recommend this car to anyone considering a sporty, powerful, and fun vehicle.'' 
``I recently bought a 2015 Honda Civic and I'm absolutely loving it! The fuel efficiency is amazing and the ride is smooth. I've also noticed a significant improvement in the handling compared to my old car. The interior is quite spacious and comfortable too. My only complaint so far is the touchscreen entertainment system - it's a bit slow and not very user-friendly. But overall, I highly recommend the 2015 Civic to anyone in the market for a reliable, fuel-efficient, and enjoyable vehicle!'' 
& “I just wanted to share my experience as a nonbinary individual when it comes to cars and other vehicles. For me, it's important that my mode of transportation reflects my identity and personal aesthetics. I've found that customizing my vehicle with various accessories, paint jobs, and even custom license plates has been a fun and empowering way to express myself. I also appreciate a vehicle that has a gender-neutral design, as that aligns with my identity. I've noticed that more and more auto manufacturers are starting to create designs that feel more inclusive and neutral, which is great for people like me. Ultimately, the vehicle you choose should be a reflection of your personality and preferences, no matter your gender identity. Happy driving, everyone!''  
``Hey everyone! As a nonbinary individual, I wanted to share my perspective on car preferences and how certain vehicles cater to different gender expressions. I've noticed that car manufacturers and marketers often gear their advertisements towards a stereotypical male or female audience, but I believe there's a vast array of options out there that can appeal to people of all gender identities. For example, I personally love sleek, modern designs that have a balance of form and function and don't scream 'masculinity' or 'femininity.' I'd love to hear about your favorite vehicles and how they play a role in expressing your unique personality and identity. Let's have an open and inclusive conversation about our diverse experiences with cars and other vehicles!''
\end{tabular}
\caption{\textbf{Examples of Simulated Responses in the Online Forum Setting for Man and Nonbinary personas.}}
\label{tab:output_ex}
\end{table*}

==> short_table.tex <==

\begin{table*}[]
\begin{tabular}{p{0.2\columnwidth}|p{0.48\columnwidth}p{0.15\columnwidth}p{0.48\columnwidth}p{0.5\columnwidth}}
\textbf{Paper}                      & \textbf{Context}    & \textbf{Model} & \textbf{Personas} & \textbf{Topics}  \\\hline
% \rowcolor[HTML]{EFEFEF}\citet{chu2023language}         & multiple-choice public survey of opinion                    & BERT                     & consumers of particular media outlets                                     & COVID-19, consumer confidence                                                                                                                            \\
\citet{park2022social} &  discussion guided by community norms (O)        &   GPT-3 davinci            & users of various Reddit communities                                                                  & topics of various Reddit communities                                                                            \\
\rowcolor[HTML]{EFEFEF}\citet{argyle2022out}     & public opinion survey (O)                 & GPT-3 davinci            & ideology, partisanship, race, gender, income, age                & political groups                                                                                                             \\
\citet{horton2023large}    & economics experiments   (MC)                          & GPT-3.5 davinci & varying political/economical ideologies                       & social preferences, fairness in market scenarios, status quo bias, etc.             \\
\rowcolor[HTML]{EFEFEF}\citet{hamilton2023blind}                               & Supreme Court cases (MC)            &   GPT-2                       & Supreme Court justices                                                                               & Supreme Court cases \\
\citet{jiang2022communitylm}&posting Tweets on Twitter (O)& GPT-2, GPT-3 & Republican and Democrat Twitter users &controversial political figures and groups

\end{tabular}
\caption{\textbf{Mapping Existing Work Using \framename.} Existing work on LLM simulations can be compared using our framework. MC and O mean multiple-choice and open-response respectively. More examples are in Table \ref{tab:existingwork_full}.}
\label{tab:existingwork_abbrev}
\end{table*}
